Bootstrapping Multilingual Semantic Parsers using Large Language Models

Despite cross-lingual generalization demonstrated by pre-trained multilingual models, the translate-train paradigm of transferring English datasets across multiple languages remains to be a key mechanism for training task-specific multilingual models. However, for many low-resource languages, the availability of a reliable translation service entails significant amounts of costly human-annotated translation pairs. Further, translation services may continue to be brittle due to domain mismatch between task-specific input text and general-purpose text used for training translation models. For multilingual semantic parsing, we demonstrate the effectiveness and flexibility offered by large language models (LLMs) for translating English datasets into several languages via few-shot prompting. Through extensive comparisons on two public datasets, MTOP and MASSIVE, spanning 50 languages and several domains, we show that our method of translating data using LLMs outperforms a strong translate-train baseline on 41 out of 50 languages. We study the key design choices that enable more effective multilingual data translation via prompted LLMs.

==> [eacl2023] mnsp-datasynth_arXiv/error_anecdotes.tex <==
\begin{table*}[!ht]
\centering
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{|l||l|}
\hline
                                     
\multirow{3}{*}{Slot Value Mismatch ($41.1\%$)} & Utterance: Set an alarm for 5 pm tomorrow                                                       \\
                                     & Prediction: {\tt [IN:CREATE\_ALARM [SL:DATE\_TIME {\color{red} for} 5 pm ] [SL:DATE\_TIME tomorrow ]  }                \\
                                     & Target:  {\tt [IN:CREATE\_ALARM [SL:DATE\_TIME 5 pm ] [SL:DATE\_TIME tomorrow ]  }                       \\ \hline\hline
\multirow{3}{*}{Wrong Intent ($19.5\%$)}        & Utterance: What can I do today                                                                             \\
                                     & Prediction:{\tt {[}IN:{\color{red}QUESTION\_NEWS} {[}SL:DATE\_TIME today {]}{]}}                                            \\
                                     & Target: {\tt {[}IN:GET\_EVENT {[}SL:DATE\_TIME today {]} {]}  }                                                  \\ \hline\hline
\multirow{3}{*}{Missing Slot ($15.1\%$)}        & Utterance: Play Justin Timberlake 's newest single                                                         \\
                                     & Prediction:{\tt {[}IN:PLAY\_MUSIC {[}SL:MUSIC\_TYPE single {]} {]}  }                                          \\
                                     & Target: {\tt {[}IN:PLAY\_MUSIC {[}SL:{\color{red}MUSIC\_ARTIST\_NAME Justin Timberlake }{]} {[}SL:MUSIC\_TYPE single {]} {]}} \\ \hline\hline
\multirow{3}{*}{Extra Slot ($14.4\%$)}          & Utterance: play music on the speaker                                                                       \\
                                     & Prediction: {\tt {[}IN:PLAY\_MUSIC {[}SL:MUSIC\_TYPE music {]} {[}SL:{\color{red}MUSIC\_TYPE speaker} {]} {]} }               \\
                                     & Target: {\tt {[}IN:PLAY\_MUSIC {[}SL:MUSIC\_TYPE music {]} {]} }                                                 \\ \hline\hline
\multirow{3}{*}{Slot Confusion ($9.9\%$)}      & Utterance: audio call wedding planner please                                                               \\
                                     & Prediction:{\tt {[}IN:CREATE\_CALL {[}SL:{\color{red} CONTACT} wedding planner {]} {]}      }                                 \\
                                     & Target: {\tt {[}IN:CREATE\_CALL {[}SL:GROUP wedding planner {]} {]} }   
                                     \\ \hline                                      
\end{tabular}
\end{adjustbox}
\caption{\textbf{Examples of Error Categories} (\S~\ref{sec:error_analysis}) The errors in the predicted parse can be broadly classified into five categories:
(i)~Slot Value Mismatch: Predicted parse has the correct signature but the slot-values are incorrect, (ii)~Wrong Intent: High-level intent of the predicted parse is incorrect, (iii)~Missing Slot: One or more slots in the gold parse do not appear in the output, (iv)~Extra Slot: Output contains extra slot(s) compared to the gold,
(v)~Slot Confusion: Prediced parse contains the correct correct intent and number of slots but the wrong slot-types.
}
\label{tab:error_examples}
\end{table*}

==> [eacl2023] mnsp-datasynth_arXiv/main_results_massive.tex <==
\subsection{Additional results}
\label{sec:app:massive}
\begin{table}[ht!]
\centering
\small
\begin{adjustbox}{width=\columnwidth}
\begin{tabular}{@{}lcccccc|c@{}}
\toprule
\multirow{2}{*}{\textbf{Lang}} & \multirow{2}{*}{\textbf{\zeroshot}} & \multirow{2}{*}{\textbf{\fewshot}} & \multirow{2}{*}{\textbf{\taf}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{\taf} + \\ \textbf{\fewshot}\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{\ours}\\ (\topk{})\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{\ours{}}\\ (\topp{})\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{\gold} \\ (skyline) \end{tabular}} \\
                      &                            &                           &                      &                                                                        &                                                                          &                                                                          &                       \\ \midrule
af   & 48.5      & 59.0       & 64.5 & 64.5        & 66.7        & 66.3        & 68.5 \\
am   & 31.0      & 47.6     & 58.3 & 57.4        & 56.1        & 55.5        & 64.6 \\
ar   & 35.9      & 50.5     & 57.2 & 58.0          & 56.6        & 57.3        & 65.5 \\
az   & 39.3      & 57.1     & 60.5 & 60.5        & 62.6        & 62.8        & 68.8 \\
bn   & 40.8      & 55.4     & 62.1 & 61.7        & 61.1        & 62.0          & 68.3 \\
cy   & 26.7      & 44.8     & 59.1 & 58.3        & 61.1        & 61.8        & 65.1 \\
da   & 57.5      & 62.4     & 66.2 & 66.3        & 69.1        & 68.5        & 71.0   \\
de   & 54.3      & 62.8     & 67.5 & 67.7        & 68.3        & 68.4        & 70.4 \\
el   & 47.3      & 57.8     & 64.2 & 65.5        & 65.2        & 65.1        & 68.7 \\
en	 & 72.7	     & 71.4	    & 73.5 & 72.9	     & 73.3	       & 73.4	     & 73.0  \\
es   & 53.4      & 58.1     & 64.6 & 64.6        & 64.7        & 64.7        & 66.6 \\
fa   & 48.8      & 58.0       & 63.1 & 62.9        & 62.8        & 63.2        & 68.1 \\
fi   & 47.5      & 58.4     & 65.0   & 65.3        & 66.7        & 67.2        & 70.9 \\
fr   & 54.6      & 58.0       & 65.3 & 64.9        & 63.9        & 63.7        & 67.1 \\
he   & 35.3      & 56.1     & 60.6 & 61.2        & 55.3        & 56.6        & 68.3 \\
hi   & 40.1      & 54.4     & 61.6 & 62.5        & 63.1        & 63.5        & 66.2 \\
hu   & 44.1      & 57.1     & 63.8 & 63.6        & 64.5        & 65.4        & 69.7 \\
hy   & 39.3      & 53.8     & 58.7 & 59.2        & 62.3        & 62.5        & 67.1 \\
id   & 55.3      & 60.2     & 65.5 & 65.9        & 66.6        & 66.0          & 69.1 \\
is   & 41.3      & 54.4     & 62.2 & 61.5        & 63.6        & 63.5        & 69.5 \\
it   & 52.3      & 58.6     & 64.0   & 63.6        & 65.2        & 65.8        & 67.2 \\
ja   & 45.6      & 55.1     & 56.3 & 56.5        & 65.6        & 65.6        & 67.3 \\
jv   & 34.3      & 51.7     & 58.6 & 60.2        & 62.0          & 61.6        & 66.7 \\
ka   & 36.5      & 53.4     & 53.5 & 54.6        & 59.2        & 59.6        & 65.7 \\
km   & 37.8      & 51.1     & 49.1 & 53.7        & 55.3        & 54.3        & 62.8 \\
kn   & 37.1      & 49.3     & 55.0   & 55.9        & 57.7        & 57.2        & 62.1 \\
ko   & 42.1      & 56.3     & 62.2 & 63.6        & 62.4        & 63.5        & 69.3 \\
lv   & 45.4      & 56.0       & 60.4 & 61.3        & 66.0          & 66.1        & 68.8 \\
ml   & 38.6      & 53.9     & 55.5 & 56.9        & 62.5        & 62.1        & 67.5 \\
mn   & 30.9      & 51.4     & 57.6 & 59.4        & 59.5        & 59.2        & 68.0   \\
ms   & 48.6      & 58.9     & 66.2 & 66.2        & 65.8        & 65.7        & 69.2 \\
my   & 38.1      & 54.9     & 60.5 & 62.3        & 61.5        & 60.6        & 69.6 \\
nb   & 55.2      & 63.0       & 67.5 & 67.7        & 67.7        & 67.4        & 71.0   \\
nl   & 53.1      & 61.2     & 67.3 & 68.5        & 68.7        & 68.5        & 70.5 \\
pl   & 50.5      & 57.4     & 61.1 & 61.4        & 62.9        & 62.5        & 65.6 \\
pt   & 54.9      & 60.3     & 65.8 & 65.7        & 66.4        & 66.9        & 68.5 \\
ro   & 51.2      & 58.8     & 65.4 & 65.0          & 64.8        & 65.1        & 68.8 \\
ru   & 42.3      & 59.4     & 63.0   & 63.1        & 66.6        & 66.2        & 69.4 \\
sl   & 46.0        & 57.8     & 63.1 & 64.0          & 65.3        & 65.4        & 68.8 \\
sq   & 41.0       & 55.4     & 60.3 & 60.4        & 62.1        & 61.7        & 67.3 \\
sv   & 57.2      & 63.1     & 69.8 & 69.6        & 69.3        & 68.9        & 72.4 \\
sw   & 35.7      & 52.3     & 57.9 & 57.5        & 60.9        & 60.6        & 65.3 \\
ta   & 37.2      & 53.0       & 55.4 & 55.7        & 60.7        & 60.9        & 65.8 \\
te   & 38.7      & 49.0       & 51.6 & 53.6        & 56.8        & 58.5        & 61.6 \\
th   & 49.4      & 60.0       & 63.5 & 66.5        & 65.2        & 65          & 71.5 \\
tl   & 48.4      & 55.7     & 64.1 & 64.2        & 65.2        & 64.8        & 67.5 \\
tr   & 46.7      & 58.5     & 63.7 & 63.4        & 62.7        & 62.8        & 69.4 \\
ur   & 38.9      & 51.2     & 60.4 & 60.6        & 62.2        & 61.9        & 64.6 \\
vi   & 46.9      & 55.1     & 59.0   & 59.2        & 63.0          & 63.3        & 67.6 \\
zhc  & 34.7      & 56.1     & 52.0   & 53.9        & 64.2        & 63.9        & 66.3 \\
zht  & 35.2      & 51.8     & 50.5 & 52.3        & 60.7        & 60.6        & 63.6 \\ \midrule
{\average}  & 43.8      & 55.9     & 61.0 & 61.6        & 63.2        & 63.2        & 67.7 \\ \bottomrule
\end{tabular}
\end{adjustbox}
\caption{EM accuracy comparison on {\massive} dataset. {\average} reports the EM accuracy averaged across the 50 non-English languages}
\label{tab:app:massive_results}
\end{table}



\begin{table}[ht!]
\centering
\small
\begin{adjustbox}{width=\columnwidth}
\begin{tabular}{@{}lcccccc|c@{}}
\toprule
\multirow{2}{*}{\textbf{Lang}} & \multirow{2}{*}{\textbf{\zeroshot}} & \multirow{2}{*}{\textbf{\fewshot}} & \multirow{2}{*}{\textbf{\taf}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{\taf} + \\ \textbf{\fewshot}\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{\ours}\\ (\topk{})\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{\ours{}}\\ (\topp{})\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{\gold} \\ (skyline) \end{tabular}} \\
                      &                            &                           &                      &                                                                        &                                                                          &                                                                          &                       \\ \midrule
de	& 54.4	& 62.8	& 75.0 &	75.1 &	73.7 &	74.0 &	78.5 \\
es	& 57.8	& 69.5	& 74.9 &	74.5 &	75.2 &	75.4 &	82.9 \\
fr	& 62.8	& 65.9	& 78.0 &	78.5 &	79.7 &	79.6 &	80.8 \\
hi 	& 42.3	& 55.3	& 63.0 &	63.9 &	72.5 &	72.3 &	78.5 \\
th	& 42.1	& 53.9	& 60.8 &	62.9 &	66.8 &	68.0 &	77.0 \\
en	& 84.1	& 84.0	& 85.2 &	85.0 &	85.2 &	85.1 &	85.4 \\
\midrule
{\average}	& 51.9	& 61.5	& 70.3 &	71.0 &	73.6 &	73.9 &	79.5 \\ \bottomrule
\end{tabular}
\end{adjustbox}
\caption{EM accuracy comparison on {\mtop} dataset. {\average} reports the EM accuracy averaged across the 5 non-English languages}
\label{tab:app:mtop_results}
\end{table}

In Table~\ref{tab:app:massive_results}, we present detailed baseline comparisons for all the 51 languages in the \massive{} dataset. {\zeroshot}, {\fewshot}, {\taf}, and {\taf}+{\fewshot} are the baselines described in Section~\ref{sec:experiments}. {\ours} represents our method with {\topk} or {\topp} sampling used while decoding the translated examples. {\gold} is the "full-shot" skyline which utilizes the original human-translated datasets (\S~\ref{sec:gold_comparison}). Table~\ref{tab:app:mtop_results} presents the same set of results for the six languages in the \mtop{} dataset. 


\subsection{Role of decoding strategy and filtering}
\label{sec:app:decoding}
In Table~\ref{tab:app:decoding_and_filtering_appendix} we present results for different decoding strategies and role of filtering inconsistent examples as discussed in Section~\ref{sec:design_choices}.

\begin{table}[h!]
\centering
\begin{adjustbox}{width=\columnwidth}
\begin{tabular}{c cccccc}
\toprule
\textbf{Decoding} & \multirow{2}{*}{\textbf{de}} & \multirow{2}{*}{\textbf{es}} & \multirow{2}{*}{\textbf{fr}} & \multirow{2}{*}{\textbf{hi}} & \multirow{2}{*}{\textbf{th}} & \multirow{2}{*}{\textbf{\average}} \\ 
\textbf{Strategy} &  &  &  &  & &  \\ \midrule
\addlinespace[1mm]
\multicolumn{1}{l}{\textbf{Greedy}}    &  71.1 &	71.7 &	72.6 &	68.1 &	66.0 &  69.9  \\
\multicolumn{1}{l}{\textbf{\;+ Filtering}}  &  72.2 &	73.5	& 74.8 &	71.5 &	67.4 &	71.9  \\
\midrule
\multicolumn{7}{l}{\textbf{{\Topk} Sampling} ($k=40$) }\\  
\small (\#samples)  &  &  &  &  &  &    \\
1 &   70.5	&	71.7  &	73.1  &	66.8  &	66.5   &  69.6  \\
2 &   72.3	&	72.7  &	75.7  &	68.7  &	67.3   &  71.3  \\
4 &   71.3	&	73.1  &	73.8  &	68.5  &	67.8   &  70.9  \\
8 &   71.1	&	72.5  &	74.2  &	69.3  &	67.5   &  70.9  \\ 
\midrule
\multicolumn{7}{l}{\textbf{ \Topk{} Sampling}  + \textbf{Filtering} ($k=40$) } \\
\small (\#samples)  &  &  &  &  &   &  \\
1 &  72.4	 &	74.4 &	78 &	70.9 &	66.1    &	72.4    \\ 
2 &  73.6 &	74.4 &	78.2 &	72.1 &	67.9   &  73.2 \\
4 &  73.4 &	75.3 &	78.8 &	71.4 &	67.1    &	73.2    \\
8 &  73.7 &		75.2 &	\textbf{79.7} &	\textbf{72.5} &	66.8    &	73.6   \\
\midrule
\multicolumn{7}{l}{\textbf{{\Topp} Sampling} ($p=0.95$)} \\  
\small (\#samples)  &  &  &  &  &  &    \\
1 &	70.1  &	71.5 &	74.3 &	66.9 &	67.2 &	70.0 \\
2 &	71.4  &	72.1 &	74.5 &	68.8 &	67.2 &	70.8 \\
4 &	71.1  &	72.8 &	76.4 &	69.0 &	66.0 &	71.1 \\
8 &	71.9  &	72.7 &	74.2 &	70.0 &	68.4 &	71.4 \\
\midrule
\multicolumn{7}{l}{\textbf{\Topp{} Sampling} + \textbf{Filtering} ($p=0.95$)} \\
\small (\#samples)  &  &  &  &  &   &  \\
1  &	72.0 &	75.2 &	78.9 &	71.6 &	\textbf{68.1} &	73.2 \\ 
2  &	73.7 &	75.2 &	79.5 &	72.0 &	67.6 &	73.6 \\ 
4  &	73.4 &	75.3 &	79.0 &	72.1 &	67.7 &	73.5 \\ 
8  &	\textbf{74.0} &	\textbf{75.4} &	79.6 &	72.3 &	68.0 &	\textbf{73.9} \\ \bottomrule

\end{tabular}
\end{adjustbox}
\caption{\textbf{Impact of decoding strategy and filtering}: Generating multiple translations per English example using {\topk} or {\topp} sampling followed by filtering inconsistent examples offers superior downstream performance compared to using greedy decoding or sampling just one translation per example.}
\label{tab:app:decoding_and_filtering_appendix}
\end{table}



==> [eacl2023] mnsp-datasynth_arXiv/main_results_mtop.tex <==


\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{l cccccc}
\toprule
\textbf{Method} & \textbf{de} & \textbf{es} & \textbf{fr} & \textbf{hi} & \textbf{th} & \textbf{\average} \\ 
\midrule
    {\zeroshot}   & 54.4    &  57.8    & 62.8   &  42.3    & 42.1 & 51.9 \\
    {\fewshot}  &  62.8    & 69.5   &    65.9 & 55.3    & 53.9   &  61.5 \\
    TAF   & 75.0    &  74.9  &  78.0    &  63.0   & 60.8   &  70.3\\ 
    TAF + {\fewshot} & \textbf{75.1}	&	74.5 &	78.5 &	63.9 &	62.9 & 71.0\\
    \midrule
    {\ours} \small{(ours)}   &  74.0       &  \textbf{75.4}  & \textbf{79.6}   &  \textbf{72.3}    & \textbf{68.0}  & \textbf{73.9} \\
    \bottomrule
\end{tabular}
}
\caption{\textbf{EM accuracy comparison on MTOP} (\S~\ref{sec:mtop_results}): Data generated using {\ours} yields better performance on $4$ out of $5$ languages in MTOP. We observe large improvements for low-resource languages hi and th.
}
\label{tab:mtop_results}
\end{table}
